My Precious Crash Data: Barriers and Opportunities in Encouraging Autonomous Driving Companies to Share Safety-Critical Data

Safety-critical data, such as crash and near-crash records, are crucial to improving autonomous vehicle (AV) design and development. Sharing such data across AV companies, academic researchers, regulators, and the public can help make all AVs safer. However, AV companies rarely share safety-critical data externally. This paper aims to pinpoint why AV companies are reluctant to share safety-critical data, with an eye on how these barriers can inform new approaches to promote sharing. We interviewed twelve AV company employees who actively work with such data in their day-to-day work. Findings suggest two key, previously unknown barriers to data sharing: (1) Datasets inherently embed salient knowledge that is key to improving AV safety and are resource-intensive. Therefore, data sharing, even within a company, is fraught with politics. (2) Interviewees believed AV safety knowledge is private knowledge that brings competitive edges to their companies, rather than public knowledge for social good. We discuss the implications of these findings for incentivizing and enabling safety-critical AV data sharing, specifically, implications for new approaches to (1) debating and stratifying public and private AV safety knowledge, (2) innovating data tools and data sharing pipelines that enable easier sharing of public AV safety data and knowledge; (3) offsetting costs of curating safety-critical data and incentivizing data sharing.

==> 89_CHI_version.tex <==
\section{Introduction}

Shared data about on-road performance, traffic incidents and protocol deviations can improve autonomous driving safety to benefit all autonomous driving developers and the public interest alike. %
Safety-critical incidents are rare and contextually specific events; aggregating data provides more for autonomous driving machine learning (ML) models to train on, thereby decreasing errors and malperformance.
Given that, we ask: What  barriers hinder autonomous driving data sharing outside organizations? How might data designers and data tool designers help?
To answer this question, we conducted an interview study with \textit{N=12} autonomous driving industry practitioners.
Our findings point out that, beyond concerns around data security and privacy, three key obstacles hinder sharing: 1) data economics that motivate possessing unique data as valuable assets, 2) lack of definition in safety-critical data, and 3) decentralized and non-standardized data collection and access protocols.
Based on these findings, we discuss changes in data collection and management, policy and incentives that can help motivate people working in automotive companies to share data to our collective mutual benefit.










\clearpage
\section{Related Work}
\hauke{Why are we not using this? There is good content here. }

\subsection{Data sharing in autonomous driving}
While much of machine learning's recent advances have been based on  shared datasets and algorithm development~\cite{ong_OpenScienceMachine_2014, vanschoren_OpenMLNetworkedScience_2014, Dickson_2022}, the autonomous driving sector has been less open. While there has been sharing of datasets to enable perception of objects which can be useful in autonomous driving---Argoverse Dataset, the Waymo Open Dataset and KITTI Dataset~\cite{argoai_Argoverse_2021, waymo_WaymoOpenDataset_2023, geiger2013vision} are notable examples, and \citet{bogdollAddatasetsMetacollectionData2023, yurtseverSurveyAutonomousDriving2020} have collected many more---the industry has not shared data that is specifically pertinent to critical incidents with autonomously driven vehicles on the road. This is in contrast to the voluntary reporting of safety events in the aviation industry \cite{bliss1999alarm,walkerRedefiningIncidentsLearn2017}, which, nowadays, can be used with classification and machine learning techniques to analyze common issues \cite{de2020classification, alkhamisi2020ensemble}.




In \citet{zhuWhatCanWe2022a}'s review of autonomous vehicle collision data, they show that there are only 3 scant datasets of autonomous driving collision incidents, all of which are based on human reports; none of the datasets with sensor data collected from autonomous vehicles intersect with safety-critical events.  There are datasets of human driving, such as the SHRP2 Naturalistic Driving Dataset \cite{hankey2016description} which have been analyzed for near crashes \cite{seacrist2020near, seacrist2018analysis}. There are also researchers staging and simulating safety critical events on vehicle testing tracks and in virtual environments to remedy the lack of naturalistic datasets~\cite{bashettyDeepCrashTestTurningDashcam2020, rocklageAutomatedScenarioGeneration2017, scanlonWaymoSimulatedDriving2021, strickland_AreYouStill_2022}. %
It is not clear that this simulated data or human data translates over to helping to recognize or characterize safety critical incidents in autonomous driving ~\cite{revell_Sim2realIssuesTransferring_2022}.



Research highlights the value of safety-critical data, which records events like crashes and near-crashes, in enhancing autonomous driving safety via machine learning models~\cite{zhuWhatCanWe2022a, chenExploringMechanismCrashes2021}.
There are two main reasons to utilize this data. First, this type of data is one of the most effective training materials for models to learn safety-oriented decision-making in high-stakes scenarios \cite{waschle_ReviewAISafety_2022}. Knowing when, where, and how these life-threatening events took place can inform the mechanisms and causes of (near) crashes, such that autonomous driving models can proactively avoid similar conditions and/or respond to such scenarios with certainty \cite{gambiGeneratingEffectiveTest2019}. %

Second, training with such data is also critical to prevent model breakdown and malperformance \cite{rabe_DevelopmentMethodologiesSafety_2021, wormann_KnowledgeAugmentedMachine_2023}. Because safety-critical events are rather scarce among all autonomous driving data, autonomous driving models have fewer instances to learn from. This means autonomous driving systems are in fact less robust and err more in these dangerous scenarios than in safe driving environments.%




\subsection{Reasons to share safety-critical data}
Based on official numbers, autonomous driving pilots have achieved human levels of safety, with crashes occurring once every 60,000 miles driven; this equates to about five years of driving for a typical human~\cite{lee_AreSelfdrivingCars_2023}. Waymo, operating primarily in Phoenix, has set an impressive benchmark in terms of crashes per mile driven~\cite{lee_AreSelfdrivingCars_2023}.

Yet, concerns arise with newer entrants into the autonomous driving space, and more challenging situations. Numerous reports capture autonomous vehicles' unpredictable behaviors, ranging from getting trapped in cement to obstructing emergency vehicles or causing harm to pets~\cite{levenson_DriverlessCarGets_2023, shakir_CruiseRobotaxiCollides_2023, bellan_WaymoSelfdrivingCar_2023}.

The consistency of safety among companies is questioned, as evidenced by Cruise's fleet reduction post-crash~\cite{associatedpress_GMCruiseAutonomous_2023}, complete shutdowns by Uber and Argo~\cite{hawkins_DriverlessCarsAren_2022}, and increasing data suggesting Tesla's autonomous modes might not be as safe as touted~~\cite{bachman_TeslaDeathsDigital_2023, sebastianblanco_ReportTeslaAutopilot_2023, siddiqui_17Fatalities736_2023}. The sharing of safety-critical data would help to enable audits of rosy company performance reports, and comparisons across companies and scenarios.


However, the sharing of safety-critical data should be motivated less by the desire to declare winners and losers in autonomous driving, and more from a desire to make autonomous driving safer across the board. In the fiercely competitive autonomous driving arena, the World Economic Forum advocates for the sharing of safety-critical data, viewing its broad societal benefits as outweighing individual company advantages~\cite{croce_this_2019}%
Collecting such data is time-intensive due to the infrequent occurrence of safety-critical events~\cite{wang_ColdStartProblem_2020};
experts worry the individualized approach to collecting safety data will lag behind the urgent need to bolster safety~\citet{koopman_AutonomousVehicleSafety_2017, ding_SurveySafetyCriticalDriving_2023}. %



\subsection{Known barriers to autonomous driving data sharing} 
\subsubsection{Privacy and security barriers}
The privacy and security implications of sharing safety-critical autonomous driving data are central concerns cited by companies why they are reluctant to share autonomous driving data. However, recent solutions that harness blockchain and IoT technologies can improve secure data sharing, storage, and access~\cite{khanLevel5AutonomousDriving2022, mollah_BlockchainInternetVehicles_2021}. In addition, novel approaches to de-identification of data also promise to ensure greater privacy during data sharing~\cite{Lobner_deidentification_2021}.
Thanks to these advancements, clearer guidelines and best practices for secure data sharing have emerged. For instance, the Federal Automated Vehicles Policy outlines cyber-security standards and promotes sharing of safety-critical data \cite{federalAutomatedVehiclesPolicy}. 

\subsubsection{Scaring customers away}
Despite advancements in secure data sharing and public advocacy, many autonomous driving companies remain hesitant. This reluctance may be linked to concerns about public perceptions and the potential damage to brand value~\cite{andersson_ValueSafetyRevealed_2005, abraham_WhatNameVehicle_2017, panagiotopoulos_EmpiricalInvestigationConsumers_2018}. %
The release of crash data can negatively affect brand image, trust, and purchasing decisions. Indeed, a study of public sentiment following 2018's Uber-pedestrian crash and a Tesla's Model X accident showed the pronounced effect of negative incidents~\cite{penmetsa_EffectsAutonomousVehicle_2021}. %

While admitting flaws in autonomous systems can impact brand reputation, participating in data sharing could also bolster public sentiment that automated driving companies are putting their interests first. %


\clearpage
\section{Methodology}
\input{tables/participants_grouped}


In the domain of human-computer interaction, understanding the intricate work practices of professionals involved in software and technology development has been the subject of extensive research~\cite{mullerHowDataScience2019, yangInvestigatingHowExperienced2018, yildirimHowExperiencedDesigners2022}. This line of inquiry has unearthed invaluable insights into human dynamics in constructing data-centric software ecosystems~\cite{passiMakingDataScience2020, passiTrustDataScience2018, chaUnlockingTacitKnowledge2023}, and improved our understanding of stringent data needs for machine learning~\cite{sambasivanEveryoneWantsModel2021, thakkarWhenMachineLearning2022, windlItNotAlways2022}. Grounded in this understanding, we interviewed \dataworker{s} to delve into their practices and perspectives, in an attempt to uncover the barriers they face to sharing safety-critical data.
To this day very few research has investigated the work practices of autonomous driving data workers. We fill this research gap in the present study.


Our investigation spanned the first half of 2023, a transformative phase in AI marked by innovations such as ChatGPT. Concurrently, the autonomous vehicle sector witnessed volatility, including layoffs at Waymo, the closure of the Argo AI venture, and ongoing delays in Tesla's self-driving package~\cite{bellan_WaymoCuts200_2023, ohnsman_ArgoAIFord_, shakir_TeslaPausesNew_2023, associatedpress_GMCruiseAutonomous_2023}. . %

\paragraph{Participant Recruitment}
\label{sec:participant_recruitement}

We targeted participants within the autonomous driving industry, especially those with extensive experience in data-driven 'design' of autonomous driving behavior. Anticipating variances between traditional vehicle manufacturers and newer Autonomous Driving Technology firms, we sought a balanced representation from both categories. Our recruitment strategies included leveraging our professional network and employing snowball sampling.
We reached out to over 40 individuals in our network, and from this group, we were able to engage twelve participants that also met our eligibility criteria. All interviewees were employed at different leading corporations or departments focused on autonomous driving development. Four participants were affiliated with universities. We did not strive for a gender-balanced sample, given that both data work and the vehicle industry remain male-dominated fields.

Through our targeted interview recruitment, we engaged \dataworker{s} with first-hand involvement in creating open autonomous driving datasets~\cite{chang_argoverse_2019, geiger_vision_2013, sun_scalability_2020, varma_idd_2019}, which are among the most cited according to \citet{bogdollAddatasetsMetacollectionData2023}.


\paragraph{Interview Procedure}
\label{sec:interview_procedure}

We conducted semi-structured interviews online, with one or two authors present per session. Before starting, we clarified our research purpose and obtained consent to record.
The interviews were divided into three sections: (1) Participants' current data use practices in autonomous vehicle design, and (2) exploring their data needs and barriers in accessing and sharing data, and (3) and ideal dataset design activity.
Initially, we delved into their current practices: the data type, scale, structure, and source, and how these influenced autonomous driving development. Participants also contrasted current versus optimal data usage, discussing motivations and barriers to ideal usage and sharing practices.
We then explored dataset challenges they faced, including data cleaning, bias handling, and annotation. Their views on the merits and challenges of good data practices and decision-making factors were discussed.
The session concluded with the ideal dataset design activity, facilitated through a virtual tool to engage participants and draw out their optimal scenarios.
Concluding each interview, we gathered details about the participants' background and experience. These sessions, lasting 50-90 minutes, were recorded and transcribed for analysis.

\paragraph{Result Analysis}
\label{sec:result_analysis}
Utilizing an iterative coding method~\cite{carpendale_AnalyzingQualitativeData_2017}, two main authors reviewed all interviews for a consistent grasp of the research. After each session, these authors engaged in open coding via a collaborative tool, extracting initial patterns about participants' data use and management desires, obstacles, and suggested practices in autonomous vehicles. These patterns were adjusted and refined as more interviews took place. The ensuing sections showcase our findings, enriched with participant quotes for clarity.

\clearpage
\section{Findings}










\subsection{Too precious to share: Safety-critical data as scarce goods in AD data economics}
\label{sec:finding_economics}


As seen across other ML-powered applied fields, data is the currency in the AD industry. Under this premise, participants commonly acknowledged that safety-critical data is particularly valuable because it takes abundant time, effort, and luck to attain such data. As a result, once AD companies possess such resources, they view such unique data as competitive advantages and have little incentive to share. Moreover, it is unclear what they would get in return, which further demotivates sharing.

\paragraph{\textbf{Three elements make precious data: time, effort, and luck.}} Participants explain that AD practitioners often deem safety-critical data as precious resources because collecting such data not only takes substantial time (due to the infrequency of these events occurring) but also relies on several (uncommon) conditions happening simultaneously. As described in this example below: %

\begin{quote}
    \quoteP[12]{If I want to cover very special scenarios, I might need to drive a long time. Just for example, with the pedestrian crossing the street at night time when it's raining, I can make [data collection happen at] the night time, but I can't make people crossing the street. [...] If I'm in California from April to November, I might not see a single day of rain.}
\end{quote}


Furthermore, there are few good substitutes for such data. Participants acknowledged that simulation is indeed often applied to generate data in need. However, safety-critical data is typically ``hard to stage and hard to simulate'' (P12) given all the dynamics evolving around these events. %


\paragraph{\textbf{Skepticism around mutual benefits of data sharing.}} Indeed, the value of safety-critical data is well-acknowledged, but we also questioned why the autonomous driving industry has not benefited from developing a shared economy mode -- as seen in the aviation industry or genetic research. Overall, participants responded with skepticism toward this concept. They often view the safety-critical data collected by their companies as unique ``case studies'' that showcase when their AD models err in the specific environments and conditions where they serve their major customers. In this regard, they are not certain whether such information would be useful to others, and they also doubt whether others' safety-alarming scenarios could be applicable and informative for their design. 

Besides, \dataworker{s} may collect specific safety-critical attributes %
just to solve a few specific model training/testing tasks. Without targeted, timely needs, practitioners are less convinced about the usefulness and usability of safety-critical data produced externally. As a result, the mutual benefits are less clear, which again discourages them from practicing data sharing more.






\subsection{Searching without names: Lack of definition of safety-critical events means larger and more haphazard data sets}
\label{sec:finding_identification}

Furthermore, participants highlighted creating safety-critical data sets takes such large amounts of work because identifying safety-critical events is difficult in the first place.
Two reasons explain this hardship:
\textit{First, these hazard instances can be hard to foresee and define in advance.} 
As a result, \dataworker{s} often have to look for ambiguously defined, rare events in large amount of data stream.
\textit{Second, \dataworker{s} constantly encounter safety-critical events occurring under unseen scenarios as AD data collection continues non-stop.} 
Given the novelty of these occurrences, it takes additional time and effort for \dataworker{s} to verify and comprehend the nature of these events, distinguishing unseen but safe driving behaviors from those that are truly life-threatening. In the following, we further elaborate on each of these aspects. %


\paragraph{\textbf{Defining safety-critical events in advance is inherently difficult}}
The causes and outcomes of hazardous driving patterns are countless. Moreover, even identical driving behaviors can lead to drastically different results in different road and traffic conditions. Predicting possibly dangerous outcomes from unseen scenarios is nothing but intractable.
While some safety-alarming patterns are straightforward to identify and can be automatically flagged, the vast majority of them are not predictable. This unpredictability can also stem from the changing nature of safety requirements and the dynamic conditions of autonomous driving.
As a result, there is currently no consensus on a standard, fixed set of safety-critical events for AD, while fatal circumstances can take place beyond one's imagination and expectations.

\begin{quote}
    \quoteP[12]{You also can never imagine all of them. So whenever I ask people to figure out what crazy things can happen, they will always only scratch the surface. So it's always, nobody could dream up. And you will never be able to get everything recorded out there}.
\end{quote}

This implies \dataworker{s} are commonly ``looking at phenomena that haven't been explored in that definition'' (P5). This makes the already labor-intensive data processing and labeling task even more onerous, because \dataworker{s} essentially need to dig out ambiguously defined, relatively rare events from a massive scale of data.

\begin{quote}
    \quoteP[3]{%
    When you're trying to figure out why something doesn't work, and you're digging into things, and you realize like, [...] the labels are slightly off, and that's what's causing the issue}.
\end{quote}


\paragraph{\textbf{\Dataworker{s} constantly encounters unseen safety-critical scenarios as data collection is always-on}}
Not only do \dataworker{s} work with enormous amounts of data, but the scale of AD data grows in a ceaseless fashion. Data collection at these AD companies continues day and night; data streams are poured into the data work pipeline non-stop. Furthermore, as ADs are tested in diverse environments, conditions, and routes, unforeseen cases often emerge. As a result, \dataworker{s} constantly encounter new events, including safety-critical instances occurring in previously unseen environments or scenarios.




While encountering these novel instances helps expand \dataworker{s}' knowledge of what counts as safety-critical events, it also takes much time and additional work for them to comprehend their causes and mechanisms. In fact, every time a driver disengages with the autonomous driving mode, an \dataworker{} would need to investigate the instance. While such disengagement can signal drivers attempting to avoid life-threatening circumstances, it can also take place when the driving condition is completely safe. Therefore, simply differentiating a dangerous case from a harmless one can already demand much work from \dataworker{s}. %
\begin{quote}
    \quoteP[12]{Whenever the safety driver had to somehow do something with the vehicle, those situations are always analyzed. So then we want to understand what happened. But there are also lower severity issues that have nothing to do with safety. Maybe someone was just feeling uncomfortable in their seat. For example, acceleration is too high or deceleration is a bit too high, or there was a slight swerving in the lanes, so anything that [makes] someone feel weird but is not vehicle- and safety-relevant. Those also take time to analyze.
    }.
\end{quote}

After recognizing a specific driving condition that could cause fatal consequences, it also takes \dataworker{s} time to verify whether similar driving behaviors or environments would consistently trigger safety concerns. In some cases, \dataworker{s} would need to see autonomous vehicles ``struggled in similar scenarios for more than 20 times'' (P7) before they reach enough evidence to proceed with further design or modeling changes. However, because these safety-critical events are rare and unique, it takes a substantial amount of time for similar ones to occur in the future. In seeking a more efficient path, \dataworker{s} often wish to sift through past events for similarities. Yet, the absence of textual records for these unique occurrences and their inherent complexity make extracting them from the existing data an uphill task.












\subsection{Decentralized and non-streamlined data workflows impede integration}
\label{sec:finding_landscape}

Finally, different practices in processing autonomous driving data within and across organizations make data sharing practically difficult. Such heterogeneity can be rooted in two ways: first, the data being collected are already different by nature; second, how these data are processed and handled also varies to a substantial degree.


\paragraph{\textbf{Highly individualized data needs cultivate different and incompatible data sets}}

To begin with, \dataworker{s} have highly individualized autonomous driving design goals and data needs. When asked about their desires for an ``ideal dataset'', our participants landed on widely different responses with what they needed to support their design. As such, they commonly believed working with data from external sources or publicly available sources could not suffice their autonomous driving design goals.












\paragraph{\textbf{Variability in access and practices}} 
Furthermore, even within the same company, \dataworker{s} work with and have access to very different types of data. 
For example, P5 described that one \dataworker{} on their team worked with scope-limited data from an individual sensor-equipped test vehicle, while most others had access to data from at least a dozen regularly deployed test vehicles. 
Depending on company and task, \dataworker{s} are positioned anywhere between working with a single stable data source, mixing various datasets to creating new data from internal data pipelines for other \dataworker{s}. 
While single use of datasets is more common in research positions, such as engineering new algorithms or studying driving behaviors, mixing and creating of new data is much more common in release-oriented autonomous driving production. Use of open-sourced data sets other than for benchmarking is rare; all interviewees rely heavily on company internal data sources, ranging from access to static databases to active shaping of data pipelines and data annotation procedures.



\paragraph{\textbf{Dumping data to the cloud first demands more work to source safety-critical information later.}}
Because pre-defining life-threatening events are rather challenging (as we discussed in Section~\ref{sec:finding_identification}), such data is seldom remarked as safety-critical when data collections take place.
Instead, practitioners suggest the practice of ``\textit{cloud dumping}'' is more common.
This means all the large amounts of data would be collected and stored to the cloud first. Afterward, \dataworker{s} would take much work to \textit{source} safety-critical information. Indeed, AD companies often have to build and manage dedicated models to identify similar data that provides safety-critical information on demand.
As P11 elaborated in an example, if the current need is to improve autopilot's capability of recognizing stop signs, \dataworker{s} would have to work through these dedicated models to source, say, more instances with stop signs from existing data.
Though this process is not impossible to accomplish, it is also not the most efficient and demands more work during the already labor-intensive data workflows.



\begin{quote}
    \quoteP[2]{People capture all the data. We call it data dumping into the cloud. That is a lot less efficient. [...] you cannot just collect millions and millions of terabytes of data, and then try to make sense out of it. So we have to be very specific about the type of information that we want}.
\end{quote}
























\clearpage
\section{Discussion}

The present work takes the initial attempt to closely examine outstanding barriers that industry practitioners face should they practice sharing safety-critical data outside of their organizations. Besides some known and speculative obstacles (i.e., concerns around security, privacy, and brand values), our interview study reveals three unique unresolved challenges: (1) data economics that deems safety-critical data as unique assets that benefit internal uses \textit{only}. (2) ambiguous definitions of safety-critical events, (3) lack of streamlined support throughout the data pipeline.




\subsection{Two needs to enable safety-critical data-sharing}

\subsubsection{Need for streamlined workflows to handle large-scale data streams}
\label{sec:finding_automation}

Across our findings, participants emphasized the onerousness of handling safety-critical data as there is no centralized and standardized approach to define, identify, and process such data. 
We see particular needs to streamline and automate various steps of autonomous driving data workflows.

\textit{We propose safety-critical events should be clearly defined in advance so that safety-critical data can be automatically remarked on the spot when data collection takes place.}
This proposal is to mitigate two current challenges: 
First, the current ``cloud-dumping first'' practice requires \dataworker{s} to spend much extra effort on retrospectively sourcing safety-critical data. 
Second, \dataworker{s} often have to look for rare and ambiguously defined data among a large number of data streams.

To realize this ideal practice, two specific action items need to be addressed. 
To begin with, we again see the need for clear definitions of safety-critical events \textit{in advance}. We further discuss the various sources of input needed to achieve this goal in the next section.
Next, every time a new type of safety-critical event is defined, there needs an automated pipeline that supports deployment. 
In this case, when the need to analyze a new safety-critical feature arises, one starts by providing a concrete definition for this (potentially) hazard event. 
Then, upon attaining internal approvals, there should be a means to automatically update specifics for data collection. 
Going forward, data collection across all autonomous vehicles will include and remark relevant attributes that capture this type of safety-critical event.

We suspect such practices can add much value to proactively recognizing safety-critical information on the spot of data collection, in contrast to the current retrospective approach to source important information afterward. 
While there are various automation tools that support different tasks throughout the autonomous driving data workflow, most of them focus on automating data processing work that occurs \textit{after} large amounts of data have already been collected.
Instead, we suggest improving efficiency by restructuring the autonomous driving data workflow.
We hope by mitigating the labor- and resource-intensive work processes, safety-critical data would be less difficult to attain.
Accordingly, we look to this shift to change practitioners' perceptions of data being too precious to share. 











\subsubsection{Need for shared definitions of safety-critical autonomous driving events}
\label{sec:need_def}

Across our findings, we see constant struggles with identifying safety-critical events from massive data streams as these unique instances are challenging to define in advance. 
Machine learning researchers have already contributed to defining these rare events from an algorithmic perspective. 
Through studying adversarial learning (i.e., learning rare instances that could attach machine learning models) and out-of-distribution machine learning, ML researchers define these special cases by how varies from given data distributions.

On the other hand, a more human-centered approach to defining safety-critical events is mostly absent at the moment.
However, as what we learned from our participants, hazard events that can be automatically flagged by machines remain limited.
At the same time, machine perceptions versus human perceptions of safety concerns can vary at a large degree.

Indeed, projecting complex conditions that jointly cause life-threatening events can be a true enigma.
Alternatively, HCI researchers and practitioners can contribute by attempting to understand users' situated experience during (near) crash scenarios. 
This can help with identifying driver behavioral patterns that can be (potentially) dangerous and defining safety-critical events that are caused by drivers' misbehavior.
Based on this human behavior insights, HCI researchers can, one on hand, start to identify universal traits that commonly lead to fatal incidents. On the other hand, new autonomous driving design proposals can help prevent such hazard behaviors from the driver's ends.






\subsection{Call for actions to the greater autonomous driving community}

To tackle these above-mentioned unresolved challenges, we call for joint efforts from researchers, designers, developers, and practitioners from the autonomous driving community to contribute to a clearer, more actionable agenda for the autonomous driving industry to practice cross-organization, cross-field sharing of safety-critical data. Below, we lay out desirable efforts by specific roles.

\begin{enumerate}
    \item Autonomous driving safety researchers can contribute by assembling and defining safety-critical events (as discussed in Section~\ref{sec:need_def}).
    \item Data work researchers can contribute by designing and developing automation tools that facilitate deployment of new safety-relevant attributes for data collection.
    \item Technology and organizational behavior researchers can contribute by outlining organizational best practices to coordinate and streamline the various steps needed to define, recognize, and handle safety-critical data.
    \item Policy researchers and practitioners can contribute in three ways: first, by setting up a common knowledge base that shares key information about autonomous driving safety-critical events and data management; second, by making reporting of hazard incidents at ease~\cite{mitchellruss_AutonomousCarDevelopers_2021,nhtsa_StandingGeneralOrder_2023}; third, by setting up new programs to assess autonomous driving safety under more precisely defined safety-critical scenarios~\cite{vanratingen_EuropeanNewCar_2016}
    \item Under this more sharing-friendly environment, autonomous driving practitioners can look to prior industry examples as case studies for benevolent sharing (e.g., Volvo's revolutionary decision in the 1950s to share its patented seatbelt design with competitors saved millions of lives~\cite{bellVolvoGiftWorld2019}; Tesla open sourcing their patented battery designs in 2014~\cite{moritz_TeslaMotorsInc_2015}.)
\end{enumerate}

Together, these efforts are expected to motivate safety-critical autonomous driving data sharing in two ways. Within organizations, these practices are expected to reduce the current practices of cloud dumping and retrospective sourcing of safety-critical information. Instead, they are expected to improve the workflows by pre-defining and identifying safety-critical events on the stop of data collection, making the workflow more efficient. Beyond single organizations, these joint efforts may shift the perceptions of safety-critical data too precious or too unique to share, encouraging data sharing even under the current autonomous driving data economics.










\subsection{Limitations}

Although we aimed for a diverse sample of industry leaders in automated vehicle behavior design, this interview study could be skewed by the interviewees we were able to engage. All participants were recruited through personal networks, as open sampling proved difficult due to companies' interest in protecting intellectual property. These interviews therefore present a Western viewpoint and exclude processes and attitudes in the East and Global South.
Moreover, the recruitment method may have inadvertently led to a selection bias, favoring participants with pre-existing connections to the research team or those who are more open to discussing proprietary practices. %
Future studies should consider employing a mixed-methods approach to address these limitations, potentially including ethnographic observation, surveys, or collaboration with experts from diverse geographical and cultural backgrounds.

\section{Conclusion}
We presented an interview study investigating incentives and barriers in sharing safety-critical autonomous driving data.
Our interviews show that the autonomous driving community, including policy makers, needs bring clarity to the definition and context of safety-critical events, inspire the creation of state-of-the-art automation tools that encompass the entirety of the data processing journey, and propose organizational strategies that foster a more collaborative and effective data-sharing environment. By addressing these pressing needs, we not only edge closer to unlocking the full potential of autonomous driving but also enhancing overall automotive safety.


==> 99_quotes.tex <==


\quoteP[6]I mean, I don't think you would see much or great barriers if you have a good point and you can show that implementing better practices solves your problem or improves your results. 
\quoteP[2]{if we had if I any, you know, magical wand, we could all come to agreement and then decide that every vehicle that is out there is contributing to solve a particular problem, right? We probably wouldn't need to use that much. This although, you know, the tools by themselves, they're useful, right?[...]
We do have new techniques that we're developing that allow these sort of untrusted collaboration to happen. It's something called federated learning. [...]
it's a way to allow learning from data, but in secure enclaves, so that you're not essentially stealing the data or sharing the data. But what you're doing is you're saying, Oh, I want to share a common solution, which is maybe a model. And then I'm going to enable that model to be training my data. And then I'm going to benefit from that, that model being improved on my data without you having to share the data. "this works in healthcare, ". But if they get an algorithm that is able to detect early cancer stages on MRIs, for example, then that's something that they both want to benefit, right. And so we come up with an agreement, and we say, we're going to run all the data and protected"with agreed processes and measurement of performance,-  by learning from these, you know, siloed data sets, then by learning only from the data that you have yourself. So this hasn't happened for automotive yet.}
\hauke{The problem is, federated learning only works, when the data does not need to be visible, the specific ML process - is static and known. And unlike healthcare the outliers are scarce, cancer is the common label.}


\quoteP[2]{ if you want your data to be protected when you're capturing it, that you can run your applications in what we call secure enclaves. Imagine, you know, when you have a computer, computers actually composed of many parts, right? You have the application that is running an operating system, is using some libraries, some firmware, and then that talks to the hardware, right? So we have solutions that we put out there, it's called SGX, that essentially creates a pipeline for your application to run in a secure enclave that goes automatically connected to the hardware, all the way to the hardware, protected all the way to the hardware, so that you make sure that whatever data you are capturing, processing, storing, gets stored on the hardware, right, on the memory that is encrypted, and only you have been able to touch and see that data, because you know, you could be, you know, running on a shared machine or something else and someone else could be copying that data, and then once that data is there and encrypted, we have ways of making our mechanisms in order to protect it also as you're transferring that data also to, let's say, your private cloud on the data center, so you do your learning. And in addition to that, we're working on other type of technologies, it's something called homomorphic encryption, because right now, whenever you collect the data and you store it, if you want to process that data, you still need to decrypt it, and then process it, and then, you know, do something with it, and then you can encrypt it again, and then, you know, you've gained some knowledge maybe. But we're working also on something called homomorphic encryption, that is a really cool concept, because it's a way of encrypting data that allows you to operate on the encrypted data without knowing what the data is, and so your data is kept confidentially. [ if you want your data to be protected when you're capturing it, that you can run your applications in what we call secure enclaves. Imagine, you know, when you have a computer, computers actually composed of many parts, right? You have the application that is running an operating system, is using some libraries, some firmware, and then that talks to the hardware, right? So we have solutions that we put out there, it's called SGX, that essentially creates a pipeline for your application to run in a secure enclave that goes automatically connected to the hardware, all the way to the hardware, protected all the way to the hardware, so that you make sure that whatever data you are capturing, processing, storing, gets stored on the hardware, right, on the memory that is encrypted, and only you have been able to touch and see that data, because you know, you could be, you know, running on a shared machine or something else and someone else could be copying that data, and then once that data is there and encrypted, we have ways of making our mechanisms in order to protect it also as you're transferring that data also to, let's say, your private cloud on the data center, so you do your learning. And in addition to that, we're working on other type of technologies, it's something called homomorphic encryption, because right now, whenever you collect the data and you store it, if you want to process that data, you still need to decrypt it, and then process it, and then, you know, do something with it, and then you can encrypt it again, and then, you know, you've gained some knowledge maybe. But we're working also on something called homomorphic encryption, that is a really cool concept, because it's a way of encrypting data that allows you to operate on the encrypted data without knowing what the data is, and so your data is kept confidentially. So you're, you can be guaranteed that your face will not, never be decrypted, but the particular application that you have agreed to use can still benefit from it, and the application still doesn't know that it's you or your data, right. It just knows that it has checked that something was, you know, correct or incorrect on encrypted data. So yeah, so homomorphic encryption is also, they call it the holy grail of data privacy. It's something that we're working on and like I said, the big problem is that it's computationally very intensive, which makes all the applications very, very slow, but we're working on accelerators to enable these to happen commercially for particular use cases, right.}

\quoteP[11]{I think you can always sign NDAs for like, you're keeping everything in-house. And of course, there's a lot of like, even within that team, it's very, you're supposed to make sure that you're not like talking too much.}

 \quoteP[2]{So the commercial fleet that we have is, I think right now, around 200 vehicles. They are deployed all around the world. So at a particular city, you might have, I don't know, maybe 10 vehicles. And they drive constantly. So we're constantly testing different routes, different type of environments, different type of weather conditions, and different times of the year with different extreme weather and things like that. Not all of that data is interesting, but when you're doing the initial testing, the initial deployments, that's when you are the most interested. Because there is always a, whenever you're deploying a solution and you think you got it, and then you go into a new location, there's always things that you think are going to work fine that you end up having to fix. Some of that information, some of that might be related to map data, for example. Oh, by the way, map data is another good example for data sets. So the type of maps that autonomous vehicles need in order to perform their behaviors are completely different than the type of maps that you're using in your Google Maps or the ones that you have right now, or you can see on the navigation systems of normal cars that are driven by human}

\quoteP[11]{I think they were using some out, they were outsourcing the labeling. But then there was a big push of keeping the data in house and also just like investing in an in house data team. And so that was the whole push where a lot of people got hired. We had our whole department is called a data annotation org, which was like at one point, like 5600 700 people, I think. And so that was a big push that was done to keep the data like in house basically. And yeah, all the team was in the US everyone was either in the in like California, so the Bay Area, or there were a few. And now I think there's more teams in Buffalo.}
\quoteP[6]{I think for companies like us, it's the incentive. You basically want, your primary driver is not increase the knowledge in the universe and share it with others. It's implementing a cool technology and sell it.}

\quoteP[10]{AYeah, I have a very unique position in that we, so I'm part of the Collaborative Safety Research Center, which is essentially externally facing group, meaning all of the stuff that we do is publicly available. I would say that, especially in the automation space, there's so many research questions and problems that open sourcing something like that leads to basically safety improvements across the board. I mean, the goal of one of our, or one of the goals of our group is to essentially motivate safety research across the industry and academia. And so if we can help academics have their research be more impactful to industry, that's a win for us. So yeah, creating those data sets helps link them more closely, I think. So again, our group is very unique in that sense. }

 \quoteP[2]{It came out of my team. And so a lot of the times we developed or we curate naturalistic driving data sets, but the events that happen in real world are not enough. And so what we do is we extract the fundamentals of what constitute those conditions, and then we enter those into a simulator so that we can generate much more synthetic data that follows that particular part. So for example, we might be interested in finding out if an algorithm can detect a dog that is following a trolley, depending on the breed, and when it's raining a lot. So we might have just one instance of that. But what we do is that when out of that situation, then we go and create using maybe Carla or some other tools internally, the variations of that condition with different intensities of rain, with different breeds, with maybe different colors or whatever. And then out of that, another data set might be created that is maybe 20\% real data, and the rest is synthetic generated data. And so those are all the types of synthetic or mixed data sets that are growing more and more because capturing the long tail end, it's a lengthy process. And we want to make sure that once we see something once, that we are then enough the system so that if any normal variation of that would be seen again in the world, that the systems are prepared to react as we consider appropriate thing. }

\quoteP[1]{Sately, that's what I need, I need to be able to make a case for the choices that I'm making. One, defend it from, you know, to management saying, hey, here is what I think is the best customer experience and here's the data to prove it. But two, more importantly, often we have questions around safety, we need to know, is it safe to, to say, allow the driver to take their eyes off the road for, or like, how often do you warn the driver, like, you know, do you let the driver, do you send an eyes off warning after five seconds, after one second, after 10 seconds, and you need data to say, hey, it may be safe to do it here because it looks like, one, people don't take their eyes off during these situations, or when it does fail, people seem to be able to react fine. And to be able to make calls like that, safety calls like that, we also need data, and it would be amazing to just be able to query that and get that immediately across all of our data sets from regular drivers. }
\quoteP[4]{Um, so this is basically raw data. So there is no, there's no labeling, for example, in terms of someone is going through, I don't know, trips and labels them. There was a critical incident that there was a takeover fail or something like this. So you, every analysis that is, that is being made on top of the data. Um, it's, it's more, more, most likely it's just run on the raw data. So you have to define yourself. If you say, for example, Um, let's say there's a single for, um, takeover request was triggered or something. Then you would need to, to, to look into data for this single. And then you, yourself would need to define your, your labels in that case. So for example, you could say, okay, it's a dangerous takeover whenever the driver. Did not touch the steering wheel. I don't know, two minutes, two seconds before the re the request was issued. Um, but there's no annotation that there is someone sitting manually annotating videos or something like this.}

\quoteP[12]{I don't remember what I said. So when the safety driver took over or disengaged, whenever the safety driver had to somehow do something with the vehicle, those situations are always analyzed. So then we want to understand what happened, was it critical to some extent. But there are also lower severity issues where something is uncomfortable. For example, acceleration is too high or deceleration is a bit too high, or there was a slight swerving in the lanes, so anything that feels somehow weird but is not vehicle relevant, those are also being analyzed. And sometimes it's just about interesting stuff. So if some specific developer wants to improve pedestrian detection, for example, then they would search for data where we have pedestrians, and maybe they want to think about incidents with pedestrians crossing a lane while it's dark and raining. So stuff like this would be like a query where they would get data, and this data would then be sorted based on how good or bad the query hits those kinds of data. }

\quoteP[1]{, I can imagine that could be extremely valuable because it's a rare event. And we can try and recreate what happened there and what kind of failures happened there or model diver behavior there and say, hey, here's the slow reaction time, or here's what they were not aware of. Here's when they took over from automation or they intervened in automation, and here's what was unsafe. That would be amazing to have that data.}

\quoteP[12]{As soon as you go to unprocessed data, you could get insight on, based on the data, how all sensors are designed.So it's hard to convince management to publish those data.
    }



\begin{quote}
    \quoteP[12]{If I want to cover very special scenarios, I might need to drive a long time. Just for example, with the pedestrian crossing the street at night time when it's raining, I can make [data collection happen at] the night time, but I can't make people crossing the street. [...] If I'm in California from April to November, I might not see a single day of rain.}
\end{quote}

\begin{quote}
    \quoteP[8]{And then the problem is over time technology progress and then the way we want to analyze the data and the parameters we want to collect is going to be very different. [...] and you need to find the document of the [data] format and how to use the data. That takes really long time. And so there are many cases [that] people started to have their own data collection instead, instead of looking into older data}.
\end{quote}    

\begin{quote}
    \quoteP[12]{You also can never imagine all of them. So whenever I ask people to figure out what crazy things can happen, they will always only scratch the surface. So it's always, nobody could dream up. And you will never be able to get everything recorded out there}.
\end{quote}

\begin{quote}
    \quoteP[3]{%
    When you're trying to figure out why something doesn't work, and you're digging into things, and you realize like, [...] the labels are slightly off, and that's what's causing the issue}.
\end{quote}

\begin{quote}
    \quoteP[2]{So we're constantly testing different routes, different type of environments, different type of weather conditions, and different times of the year with different extreme weather and things like that. Not all of that data is interesting, but when you're doing the initial testing, the initial deployments, that's when you are the most interested. Because there is always a, whenever you're deploying a solution and you think you got it, and then you go into a new location, there's always things that you think are going to work fine that you end up having to fix}.
\end{quote}   

\begin{quote}
    \quoteP[12]{Whenever the safety driver had to somehow do something with the vehicle, those situations are always analyzed. So then we want to understand what happened. But there are also lower severity issues that have nothing to do with safety. Maybe someone was just feeling uncomfortable in their seat. For example, acceleration is too high or deceleration is a bit too high, or there was a slight swerving in the lanes, so anything that [makes] someone feel weird but is not vehicle- and safety-relevant. Those also take time to analyze.
    }.
\end{quote}

\quoteP[7]{So the needle in the haystack, what would that be from your perspective? 
- Yes, yes, safety critical events. But honestly, those can be easier to find. Because with a few key parameters [...]. So I think what's more challenging to find would be. You know, I'm. ... I don't know. You know, if I'm developing a new behavior for the vehicle, I don't know, lane change or, you know, I don't know. Or like, red light scenario. There's nothing to... whereas I would like to see the top 20 times that the vehicle struggled in those scenarios or something like that. So having the database searchable with a fairly wide set of parameters. So coming up with designing that database that's easily searchable for today's problems, today's issues and then issues of the future. But knowing the unknown is a really big challenge}

\quoteP[2]{
1 need Yeah, that's a good question. I think to be honest, I think if we had if I any, you know, magical wand, we could all come to agreement and then decide that every vehicle that is out there is contributing to solve a particular problem, right? We probably wouldn't need to use that much. This although, you know, the tools by themselves, they're useful, right? If you think about it, you know, would you like to learn the from the first time that someone encounters a particular problem, right? And automatically, you know, augment that with any possible reasonable variation of that problem, and then let everybody else know about it and learn about it, right? That is the spirit of the tools that we're building today. The reality is that, you know, even even big companies with a lot of money and a lot of, you know, vehicles and customer users, right? They still only have their data. And data is something that is kept very, very privately until you have developed a data set that then you decide to put out in the open source, right? But initially, the data is something, you know, it's the new gold, because using the data, you can develop the solutions. And if you're the first to develop the solutions, it means you're the first to go to market, right? So, so the reality is that, that when you see instances, it might not be the first time that that that instance has happened in the world, it might be actually a pretty common instance, but it's the first time that you see it, right. And so you want to capture it for sure.
And you want to augment it with whichever means you have available. And until we come up to an agreement that, you know, sharing is better for everybody, then then it's difficult.
We do have new techniques that we're developing that allow these sort of untrusted collaboration to happen. It's something called federated learning. I don't know if you guys are familiar with it. But essentially, it's a way to allow learning from data, but in secure enclaves, so that you're not essentially stealing the data or sharing the data. But what you're doing is you're saying, Oh, I want to share a common solution, which is maybe a model. And then I'm going to enable that model to be training my data. And then I'm going to benefit from that, that model being improved on my data without you having to share the data. So we're doing these in other fields like healthcare, where you can think about it, you know, hospitals, they don't want to share data from patients, and they want hospital to another hospital, they also don't want to share it. But if they get an algorithm that is able to detect early cancer stages on MRis, for example, then that's something that they both want to benefit, right. And so we come up with an agreement, and we say, we're going to run all the data and protected, we're going to make sure that you know, the data cannot be stolen from you. And that is all anonymized, but we're going to learn, learn the algorithm, you've seen, we're going to let the algorithm learn using that data. And then that algorithm, that model is going to jump from all the different data sets from all the different collaborators. And then the end algorithm, the resulting algorithm, you know, it's going to be a lot more efficient than we demonstrated that you get something like, you know, 30 to 40%

}

\quoteP[12]{Any kind of misbehavior or uncomfortable reaction of the vehicle happen. It's mostly like hunting for issues more or less}.

\begin{quote}
    \quoteP[1]{There doesn't exist enough public data sets or enough data that look at the lay person's driver's behavior with an autonomous driving system. And so the kind of data sets that I look at either are from within the company, data sets from drivers that have driven within the company, or data sets that certain organizations have shared with us from our vehicles. Certain people have allowed us to collect data from their vehicles}.
\end{quote}    

\quoteP[5]{we're looking at the phenomena that hasn't been explored in that definition. [...] It could be a pet or it could be a guide dog. So we would look at a bunch of cases. We might then generate based on some of that. [..] That becomes like a training set or a golden set of a data set to compare against for then work that might come later. So we can help generate new data sets}.

\quoteP[1]{Yeah. I think the lack of intercompatibility is the primary one}.

\begin{quote}
    \quoteP[2]{People capture all the data. We call it data dumping into the cloud. That is a lot less efficient. [...] you cannot just collect millions and millions of terabytes of data, and then try to make sense out of it. So we have to be very specific about the type of information that we want}.
\end{quote}

 \quoteP[11]{Labeling efforts would get complicated (as it quickly did), and if they were having quality issues with easy labeling things like stop signs because of the communication gap with the outsourced teams, it would be a better investment to start with a smaller in house team. Because the first 10 folks who piloted the in-house team gave them better results, they ended up expanding the team. [...] And so that was the whole push where a lot of people got hired. We had our whole department is called a data annotation org, which was like at one point, like 600 700 people, I think. And so that was a big push that was done to keep the data like in house basically. And yeah, all the team was in the US everyone was either in the in like California, so the Bay Area} 

\quoteP[12]{Everybody gets their competitive advantage. I guess everybody is hoping they have the only dataset having all the secret information. [...] Those data are considered valuable. And everybody is not easily willing to share them}. 

\quoteP[12]{Recording them you need to be lucky and that makes them somehow valuable, and the question is again, do I want to publish them for free or what do I get in return?}.

\quoteP[12]{Sequences where something weird happens, really rare ones. Some recordings of like, you know, almost crashes of vehicles, for example. So, highway sequences where vehicles start drifting or turning, or like motorbikes. So, those things are hard to also simulate, especially with the dynamics and so on. So, these are really valuable data where it makes sense to to drive around and hope that something like this happens. So anything that's hard to stage, hard to simulate, [is valuable, especially when considering the] capabilities of our current algorithms in handling those kind of situations}. 

\quoteP[2]{And then we, you know, after discussing with them, we followed the same forms and formats and we put together the India driving dataset. And then now that is openly available and you can download it and use it for particular reasons, whether that's perception related or planning or whatever it is.}.
\quoteP[8]{Unless you have really good autonomous process for managing the data, the data can easily become useless because everyone needs to use the data, needs to know how to use the data. And then then in many cases in the past [...] in several university projects trying to collect naturalistic driving data for safety analysis. And then the problem is over the time technology progress and then the way we want to analyze the data and then the parameters we want to collect is going to be very different. So instead of start looking into the old data, which is missing data, not calibrated, and you need to find the document of the format and so on, takes really long time. And then there's many cases of people started to have their own data collection instead, instead of looking into older data}. 

\begin{quote}
    \quoteP[4]{So when you want to analyze a new feature, and you have not yet collected the data, you can basically say, okay, tomorrow, you go through all the legal processes and everything, and then you can deploy this this signal over the air to all the cars basically tomorrow}.
\end{quote}  

